Strategic Apple Tasting

Algorithmic decision-making in high-stakes domains often involves assigning decisions to agents with incentives to strategically modify their input to the algorithm. In addition to dealing with incentives, in many domains of interest (e.g. lending and hiring) the decision-maker only observes feedback regarding their policy for rounds in which they assign a positive decision to the agent; this type of feedback is often referred to as apple tasting (or one-sided) feedback. We formalize this setting as an online learning problem with apple-tasting feedback where a principal makes decisions about a sequence of $T$ agents, each of which is represented by a context that may be strategically modified. Our goal is to achieve sublinear strategic regret, which compares the performance of the principal to that of the best fixed policy in hindsight, if the agents were truthful when revealing their contexts. Our main result is a learning algorithm which incurs $O (\sqrt{T})$ strategic regret when the sequence of agents is chosen stochastically. We also give an algorithm capable of handling adversarially-chosen agents, albeit at the cost of $O(T^{(d+1)/(d+2)})$ strategic regret (where $d$ is the dimension of the context). Our algorithms can be easily adapted to the setting where the principal receives bandit feedback -- this setting generalizes both the linear contextual bandit problem (by considering agents with incentives) and the strategic classification problem (by allowing for partial feedback).

==> model.tex <==
\section{Model and background}\label{sec:model}


\paragraph{Notation}

\begin{itemize}
    \item $\pv{\vtheta}{1}, \pv{\vtheta}{0}$: true $\vtheta$'s for the principal's reward for actions 1 and 0 respectively.
    \item $a_t \in \{0, 1\}$: action chosen at round $t$
    \item $\pv{\hvtheta}{a}_t$: estimated reward vector for action $a \in \{0,1\}$ at round $t$.
    \item $\pv{\vtheta}{a_t^*}$: is the reward vector for the action assigned to input $\vx_t$ at round $t$ by the \emph{optimal} policy. \cpedit{We need to be careful here that the optimal policy is defined wrt the true types (i.e., it's for the strategic regret benchmark).}
    \item For the adversarial setting: $\pv{\hvtheta}{a}_*$ is the optimal discretized vector for action $a$.
    \item For the adversarial setting: $a_{t, \eps}^*$: action assigned by the optimal policy in the discretized grid set at round $t$
\end{itemize}


\section{Model and Preliminaries (OLD)}

\cpcomment{TODO: include the interaction protocol here}

\begin{figure}
    \centering
    \noindent \fbox{\parbox{\textwidth}{
    \vspace{0.1cm}
    \textbf{Interaction protocol: Contextual bandits under strategic manipulations}
    
    \vspace{-0.2cm}
    \noindent\rule{16.4cm}{0.4pt}\\
    %\noindent\rule{13.9cm}{0.4pt}\\
    For each round $t \in [T]$:
    \begin{enumerate}
        \item Decision maker publicly commits to a mapping $\pi_t: \mathcal{X} \rightarrow \mathcal{A}$. Agent $\Gamma_t$ arrives with private type $\vx_t$.
        \item Agent $t$ strategically selects context $\vx_t'$ according to Assumption \ref{ass:br}. 
        \item Decision maker observes context $\vx_t'$ and plays action $a_t = \pi_t(\vx_t')$.
        \item Decision maker receives reward $r^D_t(a_t)$ and agent receives reward $r^A(a_t)$.
    \end{enumerate}
    }}
    \caption{Description of the strategy-aware contextual bandit setting we consider, which may be viewed as a generalization of the contextual bandit problem with linear rewards.}
    \label{fig:summary}
\end{figure}


We consider a setting in which a \emph{decision maker} interacts with a sequence of $T$ strategic \emph{agents}. At each time $t \in [T]$, a new agent $\Gamma_t$ arrives with a \emph{private type} $\vx_t \in \mathcal{X} \subset [-L,L]^d$ for $L \in \mathbb{R}_+$, and presents a \emph{context} $\vx_t' \in \mathbb{R}^d$ to the decision maker. Note that it is possible for $\vx_t' = \vx_t$, but the two do not necessarily coincide. Given a context $\vx_t'$, the decision maker takes an \emph{action} $a_t$ from some set of actions $\mathcal{A}$, where $\mathcal{A} = \{1, \ldots, n\}$. For each action $a \in \mathcal{A}$, we assume that the decision maker's \emph{expected reward} $\E[r^D_t(a)] \in [-1, 1]$ is a linear function of the agent's private type. In particular, we make the following assumption on the decision maker's reward.\looseness-1


\begin{assumption}[Linearity of Rewards]\label{ass:lin}
    The decision maker reward of each arm $a \in \mathcal{A}$ at time $t$ is given by
    \begin{equation*}
        r^D_t(a) = \langle \vtheta_a, \vx_t \rangle + \varepsilon_t
    \end{equation*}
    for some $\vtheta_a \in \mathbb{R}^d$ which is unknown to the decision maker, where $\varepsilon_t$ is zero-mean sub-Gaussian noise.\looseness-1
\end{assumption}

Note that if $\vx_t' = \vx_t \; \forall t \in [T]$, our setting reduces to that of linear contextual bandits (e.g, \cite{li2010contextual, agarwal2014taming}). In contrast to the decision maker's reward, we assume that each agent's reward $r^A_t(a)$ is a function of the action alone, i.e., $r^A_t(a) = r^A(a), \forall t \in [T]$, and is known to the decision maker. %It is without loss of generality to assume that the decision maker's actions are ordered according to decreasing agent reward, i.e., $r^A(1) \geq \ldots \geq r^A(n)$.
In the personalized shopping example, a consumer's private type can be thought of as the type of customer they are (e.g., loyal customer, new customer, thrifty customer, etc.). If customers knew the online platform was going to offer them a discount based on their buying habits, they may strategically alter their short-term behavior on the platform (i.e., their context) in order to obtain the highest discount possible.\looseness-1

The decision maker's \emph{policy} $\pi_t: \mathcal{X} \rightarrow \mathcal{A}$ at time $t$ is a mapping from agent contexts to actions. In particular, the goal of the decision maker is to deploy a sequence of policies $\pi_1, \ldots \pi_T$ in order to minimize \emph{strategic regret}, which is defined as follows:

\begin{definition}[Strategic Regret]\label{def:strategic}
The expected strategic regret of a sequence of policies $\{\pi_t\}_{t=1}^T$ is defined as the cumulative expected reward of $\pi^*(\vx) := \arg \max_{a \in \mathcal{A}} \sum_{t \in [T]}\mathbb{E}[r_t^D(a)|\vx]$, the optimum-in-hindsight policy given the agents' private types, minus the cumulative expected reward of the deployed sequence of policies. Formally,\looseness-1
\begin{equation*}
\E[R_{\strat}(T)] = \sum_{t \in [T]} \underbrace{\mathbb{E}[r^D_t(\pi^*(\vx_t)) | \Gamma_t]}_{\text{reward of optimal policy given private type}} - \;\;\;\; \underbrace{\mathbb{E}[r^D_t(\pi_t(\vx_t')) | \Gamma_t]}_{\text{realized reward given context}}
\end{equation*}
\end{definition}
A decision maker with sublinear strategic regret will approach the performance of the best-in-hindsight policy if agents are \emph{not} strategic as $T \rightarrow \infty$, thereby learning to ``account'' for the strategic behavior of agents in the long run. Given the decision maker policy $\pi_t$, it is natural for an agent to choose their context in a way which maximizes their reward. Specifically, we assume that agent $\Gamma_t$ determines their context by strategically modifying their private type based on the decision maker's policy, subject to a constraint on the amount of modification which is possible. In addition to being a common assumption in the literature (e.g., \cite{chen2020learning,kleinberg2020classifiers, harris2021stateful}), this \emph{budget} constraint on the amount an agent can modify their private type reflects the fact that agents have inherent constraints on the amount of time and resources they can spend on modification.\looseness-1

\begin{definition}[Stackelberg Regret]\label{def:strategic}
The expected Stackelberg regret of a sequence of policies $\{\pi_t\}_{t=1}^T$ is defined as the cumulative expected reward of $\tilde{\pi}^*(\vx') := \arg \max_{a \in \mathcal{A}} \sum_{t \in [T]}\mathbb{E}[r_t^D(a)|\vx']$, the optimum-in-hindsight policy given that agents are strategic, minus the cumulative expected reward of the deployed sequence of policies. Formally,\looseness-1
\begin{equation*}
\E[R_{\stackel}(T)] = \sum_{t \in [T]} \underbrace{\mathbb{E}[r^D_t(\tilde{\pi}^*(\vx_t')) | \Gamma_t]}_{\text{reward of optimal policy given context}} - \;\;\;\; \underbrace{\mathbb{E}[r^D_t(\pi_t(\vx_t')) | \Gamma_t]}_{\text{realized reward given context}}
\end{equation*}
\end{definition}

\cpedit{
\begin{proposition}
For the setting we define as \emph{strategy-aware contextual bandits}, strategic regret is a \emph{stronger} performance notion compared to Stackelberg regret, i.e., $R_{\stackel}(T) \leq R_{\strat}(T)$.
\end{proposition}
}

\cpedit{
\begin{proof}
The proof follows from the definitions of the Stackelberg and the strategic regret using the fact that $\pi^*(\vx_t)$ is the optimum-in-hindsight policy given the agents' private types and the fact that the agents cannot change their type when best responding.
\begin{align*}
  \E \left[R_{\stackel}(T) \right] &= \sum_{t \in [T]} \mathbb{E}[r^D_t(\tilde{\pi}^*(\vx_t')) | \Gamma_t] -  \sum_{t \in [T]}\mathbb{E}[r^D_t(\pi_t(\vx_t')) | \Gamma_t] \\ 
  &= \sum_{t \in [T]} \mathbb{E}[r^D_t(\tilde{\pi}^*(\vx_t')) | \Gamma_t] - \sum_{t \in [T]}\E \left[r_t^D(\pi^*(\vx_t) | \Gamma_t \right] + \sum_{t \in [T]} \E \left[r_t^D(\pi^*(\vx_t) | \Gamma_t \right] - \sum_{t \in [T]} \mathbb{E}[r^D_t(\pi_t(\vx_t')) | \Gamma_t] \\
  &\leq 0 + \E \left[ R_{\strat}(T) \right]
\end{align*}
\end{proof}
}

\cpcomment{not sure if we prefer to have this as an ``assumption'' as opposed to just a definition about the agent behavior model}
\begin{assumption}[Agent Best Response]\label{ass:br}
    We assume that agent $\Gamma_t$ best-responds to the decision maker's policy $\pi_t$ in order to maximize their expected reward, subject to the constraint that their context $\vx_t'$
    is within a $\delta$-radius of their private type $\vx_t$. Formally, we assume that the agent solves the following optimization to determine their context:
    \begin{equation*}
        \begin{aligned}
            \vx_t' \in &\arg \max_{\vx' \in \mathcal{X}} \; r^A(\pi_t(\vx'))\\
            \text{s.t.} \; &\|\vx' - \vx_t \|_2 \leq \delta
        \end{aligned}
    \end{equation*}
\end{assumption}

Furthermore, we assume that if an agent is indifferent between modifying their context and not modifying, they choose not to modify. See Figure \ref{fig:summary} for a summary of the setting we consider. Finally, we conclude this section by introducing the idea of an \emph{equivalence region}, which will be useful when discussing our theoretical contributions. Roughly speaking, an equivalence region corresponds to all contexts for which a policy $\pi(\cdot)$ assigns action $a$.

\cpcomment{i included a reference to policy $\pi$ when defining the equivalence region -- helps clarify between different policies and the regions they induce}
\begin{definition}[\cpedit{$\pi$-}Equivalence region]
    An equivalence region for an action $a \in \mathcal{A}$ under policy $\pi$ is defined as the set of all contexts $\vx \in \mathcal{X}$ for which policy $\pi(\cdot)$ assigns action $a$, i.e., $\pi(\vx) = a$.
\end{definition}
For the policies we consider, each equivalence region will be a closed, convex set.

